Viral Load Inference in Non-Adaptive Pooled Testing

Medical diagnostic testing can be made significantly more efficient using pooled testing protocols. These typically require a sparse infection signal and use either binary or real-valued entries of O(1). However, existing methods do not allow for inferring viral loads which span many orders of magnitude. We develop a message passing algorithm coupled with a PCR (Polymerase Chain Reaction) specific noise function to allow accurate inference of realistic viral load signals. This work is in the non-adaptive setting and could open the possibility of efficient screening where viral load determination is clinically important.

==> commands.tex <==
%\newcommand{\param}{\underline{\boldsymbol{\vartheta}}}

%%vector
\newcommand{\pt}{\tilde{p}}
\newcommand{\avec}{\mathbf{a}}
\newcommand{\ak}{\mathbf{a}(k)}
\newcommand{\cc}{\mathbf{c}}
\newcommand{\bb}{\boldsymbol{\beta}}
\newcommand{\bhat}{\hat{\boldsymbol{\beta}}}
\newcommand{\tbb}{\tilde{\boldsymbol{\beta}}}
\newcommand{\tb}{\tilde{\beta}}
\newcommand{\bbdash}{\boldsymbol{\beta'}}
\newcommand{\dd}{\mathbf{d}}
\newcommand{\ee}{\mathbf{e}}
\newcommand{\uu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\uun}{\hat{\mathbf{u}}}
\newcommand{\vvn}{\hat{\mathbf{v}}}
\newcommand{\ww}{\mathbf{w}}
\newcommand{\xx}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\transy}{\frac{y^0}{\sqrt{b_{00}}}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\0}{\mathbf{0}}
\newcommand{\btxi}{\tilde{\boldsymbol{\xi}}}

%%matrices
\newcommand{\A}{\boldsymbol{A}}
\newcommand{\B}{\boldsymbol{B}}
\newcommand{\C}{\boldsymbol{C}}
\newcommand{\tC}{\tilde{\boldsymbol{C}}}
\newcommand{\D}{\boldsymbol{D}}
\newcommand{\EE}{\boldsymbol{E}}
\newcommand{\F}{\boldsymbol{F}}
\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\btXi}{\tilde{\boldsymbol{\Xi}}}
\newcommand{\tXi}{\tilde{\Xi}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\CChat}{\boldsymbol{\hat{C}}}
\newcommand{\I}{\mathbb{I}_p}
\newcommand{\Inp}{\mathbb{I}_{np}}
\newcommand{\M}{\boldsymbol{M}}
\newcommand{\PP}{\boldsymbol{P}}
\newcommand{\QQ}{\boldsymbol{Q}}
\newcommand{\OO}{\boldsymbol{O}}
\newcommand{\LL}{\boldsymbol{\Lambda}}
\newcommand{\Sig}{\boldsymbol{\Sigma}}
\newcommand{\Om}{\boldsymbol{\Omega}}

%%%other
\newcommand{\alphak}{\alpha_k}
\newcommand{\param}{\boldsymbol{\vartheta}}
\newcommand{\lam}{\lambda}
\newcommand{\data}{\mathcal{D}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\nhalf}{\frac{n}{2}}
\newcommand{\phalf}{\frac{p}{2}}
\newcommand{\tf}{\tilde{f}}
\newcommand{\tg}{\tilde{g}}
\newcommand{\tu}{\tilde{u}}
\newcommand{\ty}{\tilde{y}}
\newcommand{\ya}{\langle y \rangle}
\newcommand{\yaa}{\langle y^{\alpha} \rangle}
\newcommand{\zz}{\zeta}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\txi}{\tilde{\xi}}
\newcommand{\teta}{\tilde{\eta}}
\newcommand{\pg}{p^{\gamma}(t, r |u y + wy_0 + vz , \lambda) }
\newcommand{\ddd}{\mathrm{d}}
\newcommand{\td}{\tilde{d}}
\newcommand{\tD}{\tilde{D}}
\newcommand{\tDd}{(\widetilde{D-d})}
\newcommand{\indep}{\perp\mkern-10mu\perp}
\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\tS}{\tilde{S}}

%%%spacing 
\newcommand{\vsp}{\vspace*{3mm}}
\newcommand{\hsp}{\hspace*{3mm}}

%%%operators
\DeclareMathOperator*{\argmax}{argmax} % thin space, limits underneath in displays
\newcommand{\sumi}{\sum\limits_{i=1}^{N}}
\newcommand{\sumr}{\sum\limits_{r=0}^{1}}
\newcommand{\sumrd}{\sum\limits_{r'=0}^{1}}
\newcommand{\lamint}{  \prod_{r=0}^1 \{\ddd \lam_r^1, \ldots,   \ddd \lam_r^n    \}   }
\newcommand{\lp}{c + \bb . \xx}

